Learning Granger Causality from Instance-wise Self-attentive Hawkes Processes

We address the problem of learning Granger causality from asynchronous, interdependent, multi-type event sequences. In particular, we are interested in discovering instance-level causal structures in an unsupervised manner. Instance-level causality identifies causal relationships among individual events, providing more fine-grained information for decision-making. Existing work in the literature either requires strong assumptions, such as linearity in the intensity function, or heuristically defined model parameters that do not necessarily meet the requirements of Granger causality. We propose Instance-wise Self-Attentive Hawkes Processes (ISAHP), a novel deep learning framework that can directly infer the Granger causality at the event instance level. ISAHP is the first neural point process model that meets the requirements of Granger causality. It leverages the self-attention mechanism of the transformer to align with the principles of Granger causality. We empirically demonstrate that ISAHP is capable of discovering complex instance-level causal structures that cannot be handled by classical models. We also show that ISAHP achieves state-of-the-art performance in proxy tasks involving type-level causal discovery and instance-level event type prediction.

==> sections/method.tex <==
\subsection{Instance-wise Self-attentive Hawkes Processes (Original version)}

Moreover, the instance-level kernel functions no longer have type-level restrictions, which means that two event pairs sharing the same event types can have two different kernel functions depending on the sequential context. Therefore ISAHP has higher expressiveness compared with MHP. For example, synergistic effects at the type level cannot be represented using MHP, but we show that synergistic effects at the type level can be approximated using independent and additive excitation at the instance level using ISAHP. Compared with NPP based models, ISAHP itself is interpretable and no longer requires axiomatic attribution methods to perform post-training process for type-level Granger causality inference.

We express the intensity function as follows:

\begin{align}
\lambda_{x_i}(t|\mathcal{H}) & = \text{softplus}(\mu_{x_i} + \sum_{j: t_j < t} \phi_{x_i,x_j}(t-t_j))\nonumber\\
& = \text{softplus}(\mu_{x_i} + \sum_{j: t_j < t} \alpha_{x_i,x_j}\exp(-\gamma_{x_i,x_j}(t-t_j))).
\label{eq:intensity}
\end{align}

\gdk{Is any $t$, with $t_j < t$ OK? Should we further bound $t$?} 

We use the self-attention mechanism from the self-attentive Hawkes process \cite{zhang2020self} to capture the instance-level attribution and infer the parameters $\alpha_{x_i,x_j}, \gamma_{x_i,x_j}$ for the corresponding kernel function. Each event $x_j$ has the time stamp and event type information $(t_j, k_j)$. We use $\bmX \in \mathbb{R}^{M\times L}$ to represent an embedding of the event sequence, where $M$ is the dimension of the embedding, $L$ is the sequence length.

The embedding of the inputs $\bmX$ is passed through the self-attention module. The attention score $\bmA$ is:
\begin{align}
\begin{split}
&\bmA = Softmax\left(\frac{\bmQ\bmK^T}{\sqrt{M_K}}\right), \\
&where \, \bmQ = \bmX^T\bmW^Q, \bmK = \bmX^T\bmW^K \\
\end{split}
\end{align}

% \begin{align}
% \begin{split}
% &\bmA = Softmax\left(\frac{\bmQ\bmK^T}{\sqrt{M_K}}\right)\bmV, \\
% &where \, \bmQ = \bmX\bmW^Q, \bmK = \bmX\bmW^K, \bmV = \bmX\bmW^V \\
% \end{split}
% \end{align}

$\bmQ$ and $\bmK$ are the query and key matrices based on different transformations of $\bmX$. $\bmW^Q, \bmW^K \in \mathbb{R}^{M \times M_K}$, and $\bmA \in \mathbb{R}^{L \times L}$. Another embedding of inputs $\bmX$ and weight $\bmW^V \in \mathbb{R}^{M \times M_V}$ is the value matrix $\bmV=\bmX^T\bmW^V$. We can then use the instance-level hidden output $\bmA_{j,i}\bmV_{j}$ to generate $\alpha_{x_i, x_j}$ and $\gamma_{x_i, x_j}$ and the aggregated attention output $\bmS = \bmA\bmV$ to generate $\mu_{x_i}$. 

\begin{align}
\begin{split}
&\alpha_{x_i, x_j} = \text{linear}(\text{gelu}(\text{linear}(\bmA_{j,i-1}\bmV_{j}))), \\
&\gamma_{x_i, x_j} = \text{linear}(\text{gelu}(\text{linear}(\bmA_{j,i-1}\bmV_{j}))), \\
&\mu_{x_i} = \text{gelu}(\text{linear}(\bmS_{i-1})). \\
\end{split}
\end{align}
\ti{I'd suggest defining a function MLP$(\cdot)$ in general. }

\gdk{Should we have $\bmA_{i,j}$ rather than $\bmA_{j,i-1}$? Where $j=i-1$?}

\gdk{Should we have $\bmS_{j}$ rather than $\bmS_{i-1}$? (where $j=i-1$)?}

\gdk{Do these make sense (are interpretable) for $|i - j| > 1$?}

% In practice, transformer usually has multi-head attention $\bmS_1, \bmS_2, ..., \bmS_H$ which are computed based on different weights $\{W^Q_h, W^K_h, W^V_h\}^H_h=1$. The final attention output is 

% \begin{align}
% \bmS = [\bmS_1, \bmS_2,..., \bmS_H]\bmW^A
% \end{align}
% where $\bmW^A \in \mathbb{R}^{HM_V \times M}$ is the aggregation matrix.

% Assume the encoding part is a one-layer transformer, we assign the attention output $\bmS$ to be the hidden representation of all events in the input sequence $\bmH \in \mathbb{R}^{L \times M}$ where $h(t_j) = \bmH(j,:)$. Specifically, Each $h(t_j)$ is used to parameterize $K$ event type-specific intensity functions:

% \begin{align}
% \lambda_k(t|\mathcal{H}_t) = f_k\left(\alpha_k \frac{t-t_j}{t_j}+\bmw^T_k\bmh(t_j)+b_k\right).
% \label{eq:intensity}
% \end{align}

% where $\mathcal{H}_t = \{(t_j,k_j):t_j < t\}$, and $f_k(x) = \beta_k \log(1+\exp(x/\beta_k))$. In Eqn. \ref{eq:intensity}, time is defined on interval $t \in [t_j, t_{j+1})$ for event $j+1$. The overall event sequence will be:

% \begin{align}
% \lambda(t|\mathcal{H}_t) = \sum^K_{k=1} \lambda_k(t|\mathcal{H}_t)
% \label{eq:intensity_sum}
% \end{align}

For model training, we minimize the negative log-likelihood (NLL) defined in Eq.~(\ref{eq:loglikelihood}) together with regularization terms on $\bm{A}$. The final objective function is given by
\begin{align}
    \label{eq:final_objective}
    \mathrm{NLL} + \mbox{(Group lasso regularization?)} + \mbox{(L2?)}
\end{align}
\na{Description of regularization terms used, etc.} \ti{I still don't understand how it is generalized to unseen samples. How can we get sparse self-attention weights?}
%\begin{align}\sum^S_{s=1}\sum^L_{i=1} \left[-\log \lambda^s_{k^s_i}(t^s_i) + \sum^K_{k=1}\int^{t^s_i}_{t^s_{i-1}} \lambda^s_{k}(t^\prime)dt^\prime\right]\end{align}\gdk{Replace $L$ with $L_s$?}


After training, we can use the inferred $\frac{\alpha_{x_i, x_j}}{\gamma_{x_i, x_j}}$ to represent the instance-level Granger causality of event $x_j$ to event $x_i$ for any available sequences. \ti{we should define $\phi$ as the normalized exponential distribution so we can get rid of the denominator $\frac{1}{\gamma_{x_i,x_j}}$}
 The type-level Granger causality $Y_{k,k'}$ for type $k'$ to type $k$ can be calculated as follows:

\begin{align}
Y_{k,k'} = \frac{\sum^S_{s=1}\sum^{L_s}_{i=1}\sum^i_{j=1}\mathbb{I}(k^s_j=k')\mathbb{I}(k^s_i=k)\frac{\alpha_{x_i, x_j}}{\gamma_{x_i, x_j}}}{\sum^S_{s=1}\sum^{L_s}_{i=1}\sum^i_{j=1}\mathbb{I}(k^s_j=k')\mathbb{I}(k^s_i=k)}
\end{align}

\na{Remarks on the architecture referencing Fig. 1 are needed.}

\gdk{Please note that the intensity function $\lambda_{x_i}(t|\mathcal{H})$ is defined as the expected instantaneous event occurrence rate conditioned on natural filtration, so it can be expressed in units of inverse time or equivalently of frequency (e.g. $sec^{-1}$ or $Hz$). Then Equation \ref{eq:intensity} implies that terms $\alpha_{x_i, x_j}$ in the summation are expressed in units of frequency and the same should hold true for $\gamma_{x_i, x_j}$ - as the exponents $-\gamma_{x_i,x_j}(t-t_j)$ are expected to be dimensionless quantities. This means, that instance-level Granger causality defined as the quotient of two ``frequency'' terms $\alpha_{x_i, x_j}$ and $\gamma_{x_i, x_j}$, will be a dimensionless quantity as naturally expected.}


